Audio-based cough counting using independent subspace analysis

In this paper, an algorithm designed to detect characteristic cough events in audio recordings is presented, significantly reducing the time required for manual counting. Using time-frequency representations and independent subspace analysis (ISA), sound events that exhibit characteristics of coughs are automatically detected, producing a summary of the events detected. Using a dataset created from publicly available audio recordings, this algorithm has been tested on a variety of synthesized audio scenarios representative of those likely to be encountered by subjects undergoing an ambulatory cough recording, achieving a true positive rate of 76% with an average of 2.85 false positives per minute.

==> Sections/abstract_draft.tex <==
The unprecedented outbreak of novel coronavirus (COVID-19) has seen the number of confirmed cases rise beyond one million, and amongst other health-related issues, a severe and chronic cough presents itself as one of the main symptoms, and this is used by clinicians to diagnose those who have contracted the virus.
Early detection of infected individuals has become one of the main concerns of health organisations.
Although manually counting coughs has the advantage of being an accurate method of quantifying coughs, this process is time-consuming and requires considerable effort by professionals, a fact that is not feasible during a time when medical services are presently under strain.
In this paper, an algorithm designed to highlight the presence of candidate cough sounds in audio recordings is presented, significantly reducing the effort required in a manual count.
The proposed algorithm uses time-frequency representations and singular value decomposition to detect the presence of sound events that exhibit characteristics of cough sounds, and produces a summary of the recordings that highlights the events detected.
Tested on synthesised audio scenarios from publicly available audio recordings, this algorithm achieved a true positive rate of up to  \SI{87}{\percent} with an average of 2.7 false positives per minute.

==> Sections/discussion.tex <==
\section{Discussion}

==> Sections/notes.tex <==
% Chat w/ Dan. Fri 27MAR2020 

Section 1. 
Overplays the faults of the algorithtm a little too much
Positivity that exists not highlighted
ISA stuff as this is the relevant background

Useful tools:
Database/annotator tool
Summary tool
Podcasts cough removal - Descript

Title: Cough summary

%% PhD meeting 3/4/20




% DAVE: 20APR2020 9pm


what is "a" the variable used as 

a is in the range blah de blah

Chi squared 
T test

% Dataset
number of coughs present in the dataset
HIGHLIGHT THAT IS  A SINGLE PERSON IN EACH RECORDING

%%
% \begin{table}[hbtp]
%     \centering
%     \caption{Results from tests signals with $\rho_{DTC} = 0.3$ and $a=5$. Mean values highlighted in bold. }
%     \begin{tabular}{lrrr}
%         \toprule
%         \# & $r_{TP} (\%) $ & $R_{FP} (min^{-1})$ & $T_{reduced} (min)$\\
%         \midrule
% 1 & 47.37 & 14.33 & 14.63 \\ 
% 3 & 90.00 & 11.10 & 11.70 \\ 
% 4 & 80.00 & 11.67 & 12.20 \\ 
% 5 & 70.00 & 12.57 & 13.03 \\ 
% 6 & 45.00 & 12.33 & 12.63 \\ 
% 7 & 90.00 & 12.53 & 13.13 \\ 
% 8 & 55.00 & 9.13 & 9.50 \\ 
% 9 & 25.00 & 5.00 & 5.17 \\ 
% 11 & 70.00 & 13.67 & 14.13 \\ 
% 12 & 25.00 & 12.47 & 12.63 \\ 
% 13 & 80.00 & 13.77 & 14.30 \\ 
% 14 & 95.00 & 13.90 & 14.53 \\ 
% 15 & 95.00 & 4.60 & 5.23 \\ 
% 16 & 50.00 & 11.03 & 11.37 \\ 
% 18 & 95.00 & 12.70 & 13.33 \\ 
% 19 & 60.00 & 13.03 & 13.43 \\ 
% 20 & 90.00 & 6.67 & 7.27 \\ 
% 21 & 85.00 & 13.83 & 14.40 \\ 
% 22 & 85.00 & 7.47 & 8.03 \\ 
% 26 & 80.00 & 14.37 & 14.90 \\ 
% 27 & 95.00 & 12.27 & 12.90 \\ 
% 29 & 80.00 & 12.73 & 13.27 \\ 
% 31 & 90.00 & 12.77 & 13.37 \\ 
% 33 & 60.00 & 12.20 & 12.60 \\ 
% 34 & 30.00 & 8.13 & 8.33 \\ 
% 35 & 55.00 & 12.07 & 12.43 \\ 
%         \midrule
%         \textbf{Mean} & \textbf{70.09} & \textbf{11.39} & \textbf{11.86} \\
%         \bottomrule
%     \end{tabular}
%     \label{tab:results}
% \end{table}

% Chat w/ Dan


Justify +/-250ms reason. include ami paper.

Consider all detections

Goal was to see if ISA would pull out coughs, it did, not to see if it can be dome automatically

Be up front regarding that the activation functions and that the automatic methods is still required.
\begin{table}[hbtp]
    \centering
    \caption{Results from candidate time-activation function $c_1$.}
    \begin{tabular}{lrrr}
        \toprule
        \# & $r_{TP} (\%) $ & $R_{FP} (min^{-1})$ & $T (min)$\\
        \midrule
3 & 100.00 & 1.40 & 0.57 \\ 
5 & 100.00 & 0.30 & 0.38 \\ 
9 & 100.00 & 0.30 & 0.38 \\ 
11 & 100.00 & 0.30 & 0.38 \\ 
12 & 100.00 & 1.80 & 0.63 \\ 
13 & 95.00 & 3.40 & 0.88 \\ 
15 & 65.00 & 5.70 & 1.17 \\ 
16 & 95.00 & 8.80 & 1.78 \\ 
31 & 100.00 & 4.10 & 1.02 \\ 
35 & 100.00 & 0.20 & 0.37 \\ 
        \midrule
        \textbf{Mean} & \textbf{95.50} & \textbf{2.63} & \textbf{0.76} \\
        \bottomrule
    \end{tabular}
    \label{tab:results_1}
\end{table}
In \tref{tab:results_2} for the case of signal 12, a higher higher true positive ratio and a lower false positive rate was also achieved indicating more coughs correctly identified less erroneous predictions when using the candidate time-activation function $c_2$.
For the case of signal 9, there is improved performance when
\begin{table}[hbtp]
    \centering
    \caption{Results from candidate time-activation function $c_2$.}
    \begin{tabular}{lrrr}
        \toprule
        \# & $r_{TP} (\%) $ & $R_{FP} (min^{-1})$ & $T (min)$\\
        \midrule
3 & 25.00 & 6.60 & 1.18 \\ 
5 & 5.00 & 7.10 & 1.20 \\ 
9 & 40.00 & 6.20 & 1.17 \\ 
11 & 20.00 & 6.40 & 1.13 \\ 
12 & 10.00 & 5.00 & 0.87 \\ 
13 & 70.00 & 6.10 & 1.25 \\ 
15 & 45.00 & 5.50 & 1.07 \\ 
16 & 40.00 & 6.00 & 1.13 \\ 
31 & 35.00 & 6.50 & 1.20 \\ 
35 & 20.00 & 6.30 & 1.12 \\  
        \midrule
        \textbf{Mean} & \textbf{31.00} & \textbf{6.17} & \textbf{1.13} \\
        \bottomrule
    \end{tabular}
    \label{tab:results_2}
\end{table}

\begin{table}[hbtp]
    \centering
    \caption{Results from candidate time-activation function $c_3$.}
    \begin{tabular}{lrrr}
        \toprule
        \# & $r_{TP} (\%) $ & $R_{FP} (min^{-1})$ & $T (min)$\\
        \midrule
3 & 90.00 & 8.50 & 1.72 \\ 
5 & 50.00 & 8.80 & 1.63 \\ 
9 & 30.00 & 11.10 & 1.95 \\ 
11 & 80.00 & 7.50 & 1.52 \\ 
12 & 60.00 & 7.20 & 1.40 \\ 
13 & 70.00 & 7.40 & 1.47 \\ 
15 & 85.00 & 4.20 & 0.98 \\ 
16 & 65.00 & 6.90 & 1.37 \\ 
31 & 35.00 & 5.90 & 1.10 \\ 
35 & 0.00 & 11.60 & 1.93 \\ 
        \midrule
        \textbf{Mean} & \textbf{56.5} & \textbf{7.91} & \textbf{1.51} \\
        \bottomrule
    \end{tabular}
    \label{tab:results}
\end{table}
